AI-Q: Quadrature by Learned Reconstruction for the Material Point Method

The dual role of material points as carriers of constitutive history and quadrature sites couples the integration accuracy of the material point method (MPM) to the evolving particle distribution. This work introduces AI-assisted quadrature (AI-Q), a framework that separates these roles through constrained learning of a local stress-reconstruction operator. The central idea is to design reconstruction for the stress moments entering the discrete momentum balance, making the assembled internal forces the principal learning objective. Exact constant reproduction and soft affine consistency constrain the approximation, while auxiliary stress supervision regularizes modes left undetermined by force matching. The network uses the particle configuration to determine the coefficients that map particle stresses to quadrature points. Constitutive updates remain on the particles, and the same reconstruction principle applies to both full and cut cells. Numerical studies demonstrate reduced mean and high-percentile internal-force errors relative to conventional particle quadrature and classical reconstruction methods over mixed stress fields and particle configurations. These improvements carry through to the stress solution in boundary-value problems, while three-dimensional tests demonstrate compatibility with large deformation. By separating material representation from force integration, AI-Q provides a general alternative to particle quadrature and a systematic route to resolving the long-standing integration problem in MPM.

==> references.tex <==
% Ordered by first citation in the manuscript. BibTeX records are also supplied.
\begin{thebibliography}{99}
\bibitem{DLMFQuadrature}
NIST Digital Library of Mathematical Functions, Section 3.5, Quadrature,
\url{https://dlmf.nist.gov/3.5} (accessed 14 October 2026).

\bibitem{Sulsky1994}
D. Sulsky, Z. Chen, H.L. Schreyer,
A particle method for history-dependent materials,
Computer Methods in Applied Mechanics and Engineering 118 (1994) 179--196.
\href{https://doi.org/10.1016/0045-7825(94)90112-0}{doi:10.1016/0045-7825(94)90112-0}.

\bibitem{Steffen2008}
M. Steffen, R.M. Kirby, M. Berzins,
Analysis and reduction of quadrature errors in the material point method (MPM),
International Journal for Numerical Methods in Engineering 76 (2008) 922--948.
\href{https://doi.org/10.1002/nme.2360}{doi:10.1002/nme.2360}.

\bibitem{Bardenhagen2004}
S.G. Bardenhagen, E.M. Kober,
The generalized interpolation material point method,
Computer Modeling in Engineering \& Sciences 5 (2004) 477--496.
\href{https://doi.org/10.3970/cmes.2004.005.477}{doi:10.3970/cmes.2004.005.477}.

\bibitem{Wilson2021}
P. Wilson, R. W\"uchner, D. Fernando,
Distillation of the material point method cell crossing error leading to a novel quadrature-based $C^0$ remedy,
International Journal for Numerical Methods in Engineering 122 (2021) 1513--1537.
\href{https://doi.org/10.1002/nme.6588}{doi:10.1002/nme.6588}.

\bibitem{Zaheer2017}
M. Zaheer, S. Kottur, S. Ravanbakhsh, B. P\'oczos, R. Salakhutdinov, A.J. Smola,
Deep Sets,
in: Advances in Neural Information Processing Systems, vol. 30, 2017.
\href{https://proceedings.neurips.cc/paper/2017/hash/f22e4747da1aa27e363d86d40ff442fe-Abstract.html}{Publisher record}.

\bibitem{Duffy1982}
M.G. Duffy,
Quadrature over a pyramid or cube of integrands with a singularity at a vertex,
SIAM Journal on Numerical Analysis 19 (1982) 1260--1262.
\href{https://doi.org/10.1137/0719090}{doi:10.1137/0719090}.

\bibitem{Loshchilov2019}
I. Loshchilov, F. Hutter,
Decoupled weight decay regularization,
in: International Conference on Learning Representations, 2019.
\href{https://arxiv.org/abs/1711.05101}{arXiv:1711.05101}.

\bibitem{Jiang2015}
C. Jiang, C. Schroeder, A. Selle, J. Teran, A. Stomakhin,
The affine particle-in-cell method,
ACM Transactions on Graphics 34 (2015), Article 51, 1--10.
\href{https://doi.org/10.1145/2766996}{doi:10.1145/2766996}.

\bibitem{Jiang2017}
C. Jiang, C. Schroeder, J. Teran,
An angular momentum conserving affine-particle-in-cell method,
Journal of Computational Physics 338 (2017) 137--164.
\href{https://doi.org/10.1016/j.jcp.2017.02.050}{doi:10.1016/j.jcp.2017.02.050}.

\bibitem{deBoor1972}
C. de Boor,
On calculating with B-splines,
Journal of Approximation Theory 6 (1972) 50--62.
\href{https://doi.org/10.1016/0021-9045(72)90080-9}{doi:10.1016/0021-9045(72)90080-9}.
\end{thebibliography}


==> sections/21_foundation.tex <==
\section{AI-assisted quadrature for the material point method}
\label{sec:method}

The material point method separates the representation of material history from the mesh on which momentum balance is solved. This separation is central to its treatment of large motion, but it also creates a numerical integration problem: the points that carry the stress move independently of the background basis against which that stress must be integrated. The proposed AI-assisted quadrature method, denoted by AI-Q, retains the material points as the carriers of constitutive history and reconstructs their stresses at mesh-associated Gauss points. The reconstruction is trained primarily through the internal force that it produces, rather than through pointwise stress agreement alone.

We develop this choice from the underlying discretization. Section~\ref{sec:foundation} identifies where conventional finite element and material point integration differ and how the difference enters the nodal force. Section~\ref{sec:objective} then compares stress-oriented and force-oriented reconstruction. The latter is realized on structured full cells in Section~\ref{sec:full}, before extending the same formulation to cut cells in Section~\ref{sec:cut}. Training data, learning objectives, and independent evaluation are presented next, followed by integration into the explicit APIC--MPM solver. Throughout the formulation, $d$ denotes the spatial dimension, bold symbols denote vectors or matrices, and superscript $\mathsf T$ denotes transpose. The Euclidean vector norm and its induced matrix norm are denoted by $\norm{\cdot}_2$. Current-volume and current-boundary measures are written as $\dd v$ and $\dd a$; in a planar calculation, volume is understood per unit out-of-plane thickness. Dimensional choices for the numerical studies are stated with the training configurations, rather than built into the reconstruction equations.

\subsection{From continuum momentum balance to particle quadrature error}
\label{sec:foundation}

\subsubsection{Continuum problem and common spatial discretization}
\label{sec:continuum}

Let $\Omega(t)\subset\R^d$ be the material region at time $t$. Its boundary is partitioned into a prescribed-velocity part $\Gamma_v(t)$ and a prescribed-traction part $\Gamma_t(t)$. The velocity is $\vct v(\vct x,t)$, the current density is $\rho(\vct x,t)$, the Cauchy stress is the symmetric tensor $\stress(\vct x,t)$, and $\vct b(\vct x,t)$ is body force per unit mass. With outward unit normal $\vct n$, prescribed velocity $\bar{\vct v}$, and prescribed traction $\bar{\vct t}$, the balance of linear momentum is
\begin{equation}
 \begin{aligned}
 \rho\vct a&=\nabla\!\cdot\stress+\rho\vct b
       &&\text{in }\Omega(t),\\
 \vct v&=\bar{\vct v}&&\text{on }\Gamma_v(t),\\
 \stress\vct n&=\bar{\vct t}&&\text{on }\Gamma_t(t),
 \end{aligned}
 \qquad
 \vct a=\frac{D\vct v}{Dt}
 =\frac{\partial\vct v}{\partial t}+(\nabla\vct v)\vct v.
 \label{eq:strong}
\end{equation}
Here $\vct a$ is material acceleration. Introducing a virtual velocity $\vct w$ that vanishes on $\Gamma_v(t)$ and integrating the stress-divergence term by parts gives
\begin{equation}
 \int_{\Omega(t)}\rho\vct w\cdot\vct a\dd v
 =-\int_{\Omega(t)}\nabla\vct w:\stress\dd v
  +\int_{\Omega(t)}\rho\vct w\cdot\vct b\dd v
  +\int_{\Gamma_t(t)}\vct w\cdot\bar{\vct t}\dd a.
 \label{eq:weak}
\end{equation}
The gradient convention is $(\nabla\vct w)_{ab}=\partial w_a/\partial x_b$, and $\mat A:\mat B=\sum_{a,b=1}^d A_{ab}B_{ab}$ denotes double contraction. Equation~\eqref{eq:weak} is a statement about the continuum and contains no choice of particles, integration points, or mesh topology.

To discretize this equation, let $\mathcal I$ be the node-index set of a computational mesh and $N_i(\vct x)$ its scalar basis function associated with node $i$. At a fixed configuration, approximate the virtual velocity and material acceleration by
\begin{equation}
 \vct w_{\mathrm g}(\vct x)=\sum_{i\in\mathcal I}N_i(\vct x)\vct w_i,
 \qquad
 \vct a_{\mathrm g}(\vct x)=\sum_{j\in\mathcal I}N_j(\vct x)\vct a_j.
 \label{eq:gridfields}
\end{equation}
The subscript $\mathrm g$ denotes a grid representation; $\vct w_i$ and $\vct a_j$ are nodal coefficients. In particular, representing the material acceleration in this space does not identify it with the partial time derivative of a fixed-grid velocity interpolation. Since the unconstrained $\vct w_i$ are arbitrary, substitution into Eq.~\eqref{eq:weak} yields
\begin{equation}
 \sum_{j\in\mathcal I}M_{ij}\vct a_j
 =\vct f_i^{\mathrm{int}}+\vct f_i^{\mathrm{ext}},
 \label{eq:semidiscrete}
\end{equation}
with
\begin{equation}
 \begin{aligned}
 M_{ij}&=\int_{\Omega(t)}\rho N_iN_j\dd v,\\
 \vct f_i^{\mathrm{int}}&=-\int_{\Omega(t)}\stress\nabla N_i\dd v,\\
 \vct f_i^{\mathrm{ext}}&=\int_{\Omega(t)}\rho N_i\vct b\dd v
                   +\int_{\Gamma_t(t)}N_i\bar{\vct t}\dd a.
 \end{aligned}
 \label{eq:massforces}
\end{equation}
These are the consistent mass matrix, internal nodal force, and external nodal force, respectively. They provide a common variational starting point for finite element and material point discretizations. Their numerical evaluation, and the locations at which material history is retained, are where the two methods take different paths.

\subsubsection{Element-associated integration in FEM and material-associated integration in MPM}
\label{sec:femmpm}

In a conventional body-fitted finite element method, the material domain is partitioned into elements $E_e(t)$, where $e$ indexes the elements. An invertible element map $\vct\varphi_e(\vct\xi,t)$ takes a reference element $\widehat E$ to $E_e(t)$, with Jacobian $\mat J_e=\partial\vct\varphi_e/\partial\vct\xi$. If $\widehat N_{ie}$ is the restriction of $N_i$ expressed in reference coordinates, the element internal force is evaluated as
\begin{equation}
 \begin{aligned}
 \vct f_{ie}^{\mathrm{FEM}}
 &=-\sum_{q=1}^{Q_e}\widehat w_q
       \abs{\det\mat J_e(\vct\xi_q,t)}\,
       \stress_{eq}\,
       \mat J_e(\vct\xi_q,t)^{-\T}
       \nabla_{\!\xi}\widehat N_{ie}(\vct\xi_q),\\
 \vct x_{eq}&=\vct\varphi_e(\vct\xi_q,t).
 \end{aligned}
 \label{eq:femquadrature}
\end{equation}
Here $Q_e$ is the number of quadrature points, $\vct\xi_q$ and $\widehat w_q$ are their reference coordinates and weights, and $\stress_{eq}$ is the constitutively updated stress at $\vct x_{eq}$. The quadrature coordinates remain fixed relative to the element even when the element moves or deforms. Consequently, the integration rule is chosen for the element-local basis and geometry, and its moments do not change because an integration point independently migrates into a neighboring element. Gaussian quadrature can be algebraically exact for suitable polynomial integrands; nonlinear stresses and nonaffine mappings still require an accuracy assessment~\cite{DLMFQuadrature}. The comparison is therefore not between an exact FEM and an inexact MPM, but between two different ways of controlling the integration rule.

MPM instead carries position, stress, and constitutive history on moving material points, while using a background mesh to calculate forces and velocity gradients~\cite{Sulsky1994}. Let $\mathcal P$ be the particle-index set. Particle $p$ has position $\vct x_p$, current volume $V_p>0$, constant mass $m_p$, and stress $\stress_p$. The standard point-particle quadrature replaces volume integrals by
\begin{equation}
 \int_{\Omega(t)}\phi(\vct x)\dd v
 \approx\sum_{p\in\mathcal P}V_p\phi(\vct x_p),
 \qquad
 \int_{\Omega(t)}\rho\phi(\vct x)\dd v
 \approx\sum_{p\in\mathcal P}m_p\phi(\vct x_p),
 \label{eq:particlequadrature}
\end{equation}
for a scalar-, vector-, or tensor-valued integrand $\phi$. In particular,
\begin{equation}
 \vct f_i^{\MPM}
 =-\sum_{p\in\mathcal P}V_p\stress_p\nabla N_i(\vct x_p).
 \label{eq:particleforce}
\end{equation}
The same particle integration gives $M_{ij}^{\mathrm P}=\sum_p m_pN_i(\vct x_p)N_j(\vct x_p)$. Applying row-sum mass lumping and using partition of unity, $\sum_jN_j(\vct x_p)=1$, gives the nodal mass used by the explicit solver:
\begin{equation}
 m_i=\sum_jM_{ij}^{\mathrm P}
     =\sum_{p\in\mathcal P}m_pN_i(\vct x_p),
 \qquad
 m_i\vct a_i=\vct f_i^{\MPM}+\vct f_i^{\mathrm{ext}}.
 \label{eq:lumped}
\end{equation}
The external force in the last equation is understood to use the selected body-force and traction discretizations. Mass lumping is a separate approximation from the internal-force quadrature and will be left unchanged in AI-Q.

Material volumes are not arbitrary fitting weights. If $V_p^0$ and $\rho_p^0$ are reference volume and density, and $\mat F_p=\partial\vct x/\partial\vct X$ is the deformation gradient at the particle, then $m_p=\rho_p^0V_p^0$ and $V_p=J_pV_p^0$, where $\vct X$ is a reference coordinate and $J_p=\det\mat F_p>0$. A solver that stores Kirchhoff stress $\mat\tau_p=J_p\stress_p$ therefore uses the identical product $V_p^0\mat\tau_p=V_p\stress_p$ in Eq.~\eqref{eq:particleforce}. AI-Q will reconstruct Cauchy stress and integrate it with current-volume weights. Normalizing a neural input must not change these physical stress--volume pairings.

\subsubsection{How the moving quadrature enters the internal-force error}
\label{sec:particleerror}

The integrand in Eq.~\eqref{eq:particleforce} is not stress alone, but stress multiplied by the gradient of a mesh basis function. A material point may continue to represent its material history accurately while becoming a poor quadrature location for this product. To isolate these effects, write the numerical particle stress as $\stress_p=\stress(\vct x_p)+\mat\epsilon_p$, where $\mat\epsilon_p$ denotes its deviation from a chosen smooth reference stress field. Subtracting the continuum internal force gives the exact decomposition
\begin{equation}
 \begin{aligned}
 \vct f_i^{\MPM}-\vct f_i^{\mathrm{int}}
 ={}&-\sum_pV_p\mat\epsilon_p\nabla N_i(\vct x_p)\\
 &+\left[\int_{\Omega(t)}\stress\nabla N_i\dd v
       -\sum_pV_p\stress(\vct x_p)\nabla N_i(\vct x_p)\right].
 \end{aligned}
 \label{eq:mpmerror}
\end{equation}
The first term propagates errors already present in the particle states. The bracketed term is a quadrature error and remains even when every particle stress is exact. Improving a constitutive update or plotting a smoother particle stress field cannot, by itself, remove this second contribution.

The local structure of that contribution can be made explicit without considering a material boundary. Take a completely filled, convex background cell $K_c$, with centroid $\vct x_c$ and particle set $\mathcal P_c=\{p:\vct x_p\in K_c\}$. The index $c$ labels background cells, and $\abs{K_c}$ is the cell volume. Define the vector-valued force integrand $\vct g_i=\stress\nabla N_i$ and the zeroth and first particle-moment defects
\begin{equation}
 \Delta m_{0,c}=\sum_{p\in\mathcal P_c}V_p-\abs{K_c},
 \qquad
 \vct{\Delta m}_{1,c}
   =\sum_{p\in\mathcal P_c}V_p(\vct x_p-\vct x_c).
 \label{eq:particlemoments}
\end{equation}
The exact first volume moment about the centroid is zero. If $\vct g_i$ is twice continuously differentiable within this cell, Taylor expansion about $\vct x_c$ gives
\begin{equation}
 \begin{aligned}
 \vct E_{ic}^{\mathrm{quad}}
 &:=-\sum_{p\in\mathcal P_c}V_p\vct g_i(\vct x_p)
                +\int_{K_c}\vct g_i(\vct x)\dd v\\
 &=-\vct g_i(\vct x_c)\Delta m_{0,c}
   -\nabla\vct g_i(\vct x_c)\vct{\Delta m}_{1,c}
   +\vct r_{ic},
 \end{aligned}
 \label{eq:momenterror}
\end{equation}
where the remainder $\vct r_{ic}$ collects second- and higher-order variation. If $M_{g,2,c}$ bounds the induced norm of the second derivative of $\vct g_i$ on $K_c$, then
\begin{equation}
 \norm{\vct r_{ic}}_2\le\frac{M_{g,2,c}}2
 \left[\int_{K_c}\norm{\vct x-\vct x_c}_2^2\dd v
       +\sum_{p\in\mathcal P_c}V_p\norm{\vct x_p-\vct x_c}_2^2\right].
 \label{eq:momentremainder}
\end{equation}
Thus matching total material volume does not suffice: the volume distribution must also match the moments required by $\stress\nabla N_i$. Even if total particle volume agrees with the volume of the entire body, the volumes assigned by particle centers to an individual background cell need not sum to that cell's volume. Transport changes both this assignment and the higher moments. Adding particles can improve coverage, but the relevant issue is the integration quality of their locations and volumes, not the count alone.

A one-dimensional constant-stress example illustrates the first defect particularly clearly. Let an interior linear basis function rise with slope $1/h$ on its left cell and fall with slope $-1/h$ on its right cell, both of length $h$. For uniform stress $\sigma_0$, the exact contributions cancel. If $\widetilde V_L$ and $\widetilde V_R$ are the sums of particle volumes assigned to those two cells, however, then
\begin{equation}
 f_i^{\mathrm{int}}=0,
 \qquad
 f_i^{\MPM}=\frac{\sigma_0}{h}
                 (\widetilde V_R-\widetilde V_L).
 \label{eq:constantcounterexample}
\end{equation}
The numerical force is nonzero whenever the two discrete volume sums differ, although no error has been introduced into the particle stresses. This example diagnoses a quadrature inconsistency; it does not imply that constant stress should produce zero force at every individual cell node or at a loaded physical boundary.

A related mechanism occurs when a particle crosses a location at which $\nabla N_i$ is discontinuous. Keeping its volume and stress continuous during the crossing, the limiting jump in its force contribution is
\begin{equation}
 \llbracket\vct f_{ip}\rrbracket
 =-V_p\stress_p\llbracket\nabla N_i\rrbracket,
 \qquad
 \llbracket\psi\rrbracket:=\psi^{+}-\psi^{-},
 \label{eq:crossing}
\end{equation}
where $+$ and $-$ denote the two one-sided limits. The influence of basis regularity on MPM integration and cell-crossing error is well documented~\cite{Steffen2008,Bardenhagen2004,Wilson2021}. A smoother B-spline gradient removes this particular jump, but it does not enforce the moment conditions in Eq.~\eqref{eq:particlemoments}. Conversely, cells intersected by a material boundary present an additional geometric difficulty because the integration domain is only a portion of the background cell. These observations motivate separating material-state storage from force integration, while keeping basis regularity, integration accuracy, and boundary geometry as distinct parts of the method.


==> sections/22_objective.tex <==
\subsection{From stress recovery to force-oriented reconstruction}
\label{sec:objective}

\subsubsection{Restoring mesh-associated quadrature}

The preceding discussion suggests using a quadrature rule attached to the background mesh, as in element integration, without transferring constitutive history away from the material points. Consider first a full cell $K_c$. Let $\mathcal I_c$ be the set of basis functions that are nonzero in the interior of $K_c$, let $N_{b,c}=\abs{\mathcal I_c}$ be its number of active nodes, and let $P_c=\abs{\mathcal P_c}$ be its particle count. A prescribed full-cell rule has $Q_{\full}$ points $\vct x_{cq}$ and positive physical weights $W_{cq}$, where $q=1,\ldots,Q_{\full}$. If the stress were available at these points, the cell force would be
\begin{equation}
 \vct f_{ic}^{\Gauss,\full}[\stress]
 =-\sum_{q=1}^{Q_{\full}}W_{cq}\stress(\vct x_{cq})
                                      \nabla N_i(\vct x_{cq}).
 \label{eq:gausstarget}
\end{equation}
Square brackets indicate the stress field supplied to the quadrature. This is a discrete Gauss force, not a claim that the corresponding continuum integral is exact. The rule now resolves the mesh-local integrand at prescribed locations; the remaining task is to infer its stress values from the available material samples.

AI-Q represents that inference by a geometry-dependent matrix $\mat R_c^{\full}\in\R^{Q_{\full}\times P_c}$:
\begin{equation}
 \widehat\stress_{cq}^{\full}
 =\sum_{p\in\mathcal P_c}R_{cqp}^{\full}\stress_p,
 \qquad
 \mat R_c^{\full}=\mathcal N_{\theta_{\full}}(\mathcal G_c).
 \label{eq:genericreconstruction}
\end{equation}
The hat denotes a reconstructed stress, $\mathcal G_c$ denotes the geometric inputs, and $\theta_{\full}$ denotes the full-cell network parameters. The same scalar coefficient $R_{cqp}^{\full}$ acts on every component of $\stress_p$. The network is nonlinear in geometry but the resulting transfer is linear in stress. It therefore retains stress superposition at fixed geometry and does not require a constitutive model to be learned. The Gauss points are evaluation sites, not additional material points with their own deformation or history variables.

We use a structured Cartesian mesh in this study because its reference geometry and basis restrictions are shared by all interior cells. The reconstruction--integration principle itself does not require a structured mesh. For an unstructured cell with an invertible reference map $\vct\varphi_c$, its Jacobian $\mat J_c$, reference query $\vct\xi_q$, reference weight $\widehat w_q$, and reference basis restriction $\widehat N_{ic}$, the corresponding ingredients are
\begin{equation}
 \begin{aligned}
 \vct x_{cq}&=\vct\varphi_c(\vct\xi_q),
 &W_{cq}&=\widehat w_q\abs{\det\mat J_c(\vct\xi_q)},\\
 \nabla N_i(\vct x_{cq})
 &=\mat J_c(\vct\xi_q)^{-\T}\nabla_{\!\xi}\widehat N_{ic}(\vct\xi_q).
 \end{aligned}
 \label{eq:unstructured}
\end{equation}
Equations~\eqref{eq:gausstarget}--\eqref{eq:genericreconstruction} then have the same form, with cell geometry included in $\mathcal G_c$ and an appropriate rule for each element type. This is an extension of the formulation, not an assertion that a network trained on Cartesian cells can be used unchanged on arbitrary elements. In particular, the geometric features, training distribution, and physical-coordinate consistency conditions must match the chosen mesh. The structured construction below fixes these choices for the present calculations.

\subsubsection{Why stress agreement and force agreement are different objectives}
\label{sec:forcechoice}

There are two natural ways to determine the reconstruction coefficients. A stress-oriented approach seeks agreement between reconstructed and reference stresses at the queries, and only afterwards evaluates the nodal force. A force-oriented approach instead judges the same reconstruction by the force it produces through Eq.~\eqref{eq:gausstarget}. The distinction is a choice of approximation objective, not a choice between maintaining stresses and discarding them.

To express it precisely, let $\vct s=\operatorname{sv}(\stress)\in\R^{n_\sigma}$ collect the independent components of a symmetric tensor, where $n_\sigma=d(d+1)/2$. The diagonal components are listed first, followed by upper-triangular components in lexicographic order; shear components are not multiplied by two. Let $\mat S_c^{\mathrm P}\in\R^{P_c\times n_\sigma}$ and $\mat S_c^{\Gauss}\in\R^{Q_{\full}\times n_\sigma}$ contain the particle and reference query stresses as rows. Then
\begin{equation}
 \widehat{\mat S}_c^{\full}=\mat R_c^{\full}\mat S_c^{\mathrm P},
 \qquad
 \vct e_c=\vvec\!\left(\widehat{\mat S}_c^{\full}-\mat S_c^{\Gauss}\right),
 \qquad
 \widehat{\vct f}_c^{\full}-\vct f_c^{\Gauss,\full}
       =\mat B_c\vct e_c.
 \label{eq:forceoperator}
\end{equation}
Here $\vvec$ stacks matrix columns, $\widehat{\vct f}_c^{\full}$ and $\vct f_c^{\Gauss,\full}$ stack the $d$ force components at all $N_{b,c}$ active nodes in a fixed order, and $\mat B_c\in\R^{dN_{b,c}\times Q_{\full}n_\sigma}$ is the known linear assembly matrix defined by Eq.~\eqref{eq:gausstarget}. It contains the Gauss weights, background-basis gradients, tensor-component placement, and the internal-force sign. No part of $\mat B_c$ is learned.

Let $\mat W_{\sigma,c}$ be a positive diagonal matrix that specifies a chosen query-stress metric, such as equal component weighting or volume weighting. Before normalization, the two approximation criteria have the form
\begin{equation}
 J_{\sigma,c}=\vct e_c^{\T}\mat W_{\sigma,c}\vct e_c,
 \qquad
 J_{f,c}=\norm{\mat B_c\vct e_c}_2^2
        =\vct e_c^{\T}\mat B_c^{\T}\mat B_c\vct e_c.
 \label{eq:twocriteria}
\end{equation}
They need not rank two candidate reconstructions in the same order. Stress errors are combined with different basis-gradient directions and quadrature weights before they become nodal forces; some components reinforce one another, whereas others cancel. Thus minimizing an unweighted stress error is not equivalent to minimizing the force error. A useful one-sided relation is
\begin{equation}
 \norm{\widehat{\vct f}_c^{\full}-\vct f_c^{\Gauss,\full}}_2
 \le\norm{\mat B_c\mat W_{\sigma,c}^{-1/2}}_2
               \sqrt{J_{\sigma,c}},
 \label{eq:stressforcebound}
\end{equation}
where the matrix norm is the induced Euclidean norm. Accurate stresses are sufficient to control the force for a bounded assembly operator, but the size and orientation of the stress error relative to that operator also matter.

The converse is more restrictive. Any nonzero error in the null space of $\mat B_c$ changes the recovered stress without changing the assembled force. Consequently, a force-only objective can leave stress modes poorly determined. This observation motivates the adopted compromise: the primary objective is agreement of the assembled internal force, with an auxiliary stress-reconstruction term and explicit consistency conditions. The precise normalizations and weights are given in Section~\ref{sec:losses}; Eq.~\eqref{eq:twocriteria} compares the underlying error measures and does not prescribe an additional training stage.

The resulting method is therefore a force-oriented stress reconstruction, not a black-box prediction of nodal forces. Substituting Eq.~\eqref{eq:genericreconstruction} into the quadrature gives an equivalent particle-to-force representation,
\begin{equation}
 \begin{aligned}
 \widehat{\vct f}_{ic}^{\full}
  &=-\sum_{p\in\mathcal P_c}\stress_p\vct g_{icp}^{\mathrm{eff}},\\
 \vct g_{icp}^{\mathrm{eff}}
  &=\sum_{q=1}^{Q_{\full}}W_{cq}R_{cqp}^{\full}
                                  \nabla N_i(\vct x_{cq}).
 \end{aligned}
 \label{eq:effectivegradient}
\end{equation}
The effective vector $\vct g_{icp}^{\mathrm{eff}}$ has units of length to the power $d-1$ and replaces $V_p\nabla N_i(\vct x_p)$ in the force mapping. It need not be formed explicitly in the implementation. This factorization explains how the network corrects the integration while the physical assembly remains known. It also preserves a common reconstructed stress for all nodes of a cell, a structure that will be important for internal-force balance.


==> sections/23_full.tex <==
\subsection{Constrained reconstruction on structured full cells}
\label{sec:full}

\subsubsection{Reconstruction domain and prescribed quadrature}

We now specialize the general construction to a uniform Cartesian background mesh with spacing $h$ in every coordinate direction. The basis degree is $k$, with $k=1,2,3$ denoting linear, quadratic, and cubic cardinal B-splines. A reconstruction cell $K_c$ is one tensor-product polynomial knot span, not the entire support of a basis function. Accordingly, the active set in Section~\ref{sec:objective} has $N_{b,c}=(k+1)^d$ nodes on an interior span. The basis definitions and node-index conventions are collected in \ref{app:basis}.

This distinction between a span and a support is essential for locality. The particle set $\mathcal P_c$ contains only particles whose current positions belong to $K_c$, even when an active basis function also extends into adjacent cells. After reconstruction, the cell force is assembled to all nodes in $\mathcal I_c$. Neighboring particles are not added to the reconstruction merely because the background basis has a wider support. A half-open ownership convention assigns a particle on a span face to one cell and prevents duplicate contributions.

For a span centered at $\vct x_c$, define its reference coordinates and coordinate transformation by
\begin{equation}
 K_c=\vct x_c+\frac h2[-1,1]^d,
 \qquad
 \vct\xi=\frac2h(\vct x-\vct x_c),
 \qquad
 \nabla_{\!x}N_i=\frac2h\nabla_{\!\xi}\widehat N_{ic}.
 \label{eq:localcoordinates}
\end{equation}
The closure is used in the displayed geometric definition; ownership on shared faces follows the half-open convention. For the centered quadratic cardinal basis, spans are shifted by half a grid spacing relative to the ordinary intervals between grid nodes. In one coordinate, the span containing $x$ is indexed by $j_0=\lfloor x/h-1/2\rfloor$ and extends from $(j_0+1/2)h$ to $(j_0+3/2)h$, with active nodes $j_0,j_0+1,j_0+2$. This index describes the physical polynomial pieces of the basis; it does not shift the mechanical nodes or the particles.

Let $g_{\full}$ be the number of one-dimensional Gauss--Legendre points on $[-1,1]$. Denote their coordinates and weights by $\zeta_a$ and $w_a$, $a=1,\ldots,g_{\full}$. A query index $q$ enumerates the tuple $(a_1,\ldots,a_d)$ and defines
\begin{equation}
 \begin{aligned}
 Q_{\full}&=g_{\full}^{\,d},
 &\vct\xi_q&=(\zeta_{a_1},\ldots,\zeta_{a_d})^{\T},\\
 \vct x_{cq}&=\vct x_c+\frac h2\vct\xi_q,
 &W_{cq}&=(h/2)^d\prod_{b=1}^d w_{a_b}.
 \end{aligned}
 \label{eq:fullrule}
\end{equation}
Thus $\sum_qW_{cq}=h^d$, independently of the number and arrangement of particles. The rule order is fixed with the selected model. In particular, $P_c$ need not equal $Q_{\full}$ and may be either smaller or larger. A Gauss rule has polynomial exactness properties for a prescribed integrand, but increasing its order cannot by itself improve the unknown stresses supplied to it. Reconstruction and quadrature accuracy must therefore be assessed separately.

\subsubsection{Geometry-conditioned reconstruction coefficients}

The full-cell input for particle $p$ consists of its local position $\vct\xi_{cp}=2(\vct x_p-\vct x_c)/h$ and relative volume
\begin{equation}
 \nu_{cp}^{\full}=\frac{V_p}{\sum_{r\in\mathcal P_c}V_r},
 \qquad
 \vct z_{cp}^{\full}=[\vct\xi_{cp},\nu_{cp}^{\full}].
 \label{eq:fullfeatures}
\end{equation}
Brackets in a feature definition denote concatenation. In the offline full-cell bank, the particle volumes sum to the model-cell volume, so this expression coincides with normalization by that volume. Online, the adapter constructs a separate input tensor with the same normalization. It does not rescale the physical volumes, masses, or Gauss weights. The normalized volume is a descriptor of relative particle representation, not a correction of the moment defect in Eq.~\eqref{eq:particlemoments}.

A shared particle encoder $\Phi_{\theta_{\full}}$ maps this input to a vector $\vct e_{cp}^{\full}\in\R^{d_{\mathrm f}}$, where $d_{\mathrm f}$ is the feature width. The encoded particles are combined into a cell descriptor by mean pooling, sum pooling, and an explicit particle count:
\begin{equation}
 \begin{aligned}
 \vct e_{cp}^{\full}&=\Phi_{\theta_{\full}}(\vct z_{cp}^{\full}),\\
 \vct u_c^{\full}&=\left[
  \frac1{P_c}\sum_p\vct e_{cp}^{\full},\quad
  \sum_p\vct e_{cp}^{\full},\quad P_c/P_{\max}\right].
 \end{aligned}
 \label{eq:pooling}
\end{equation}
Here and below, unqualified particle sums in a cell formula run over $\mathcal P_c$, and $P_{\max}$ is the array capacity. Shared encoding and order-independent pooling follow the set-network construction of Deep Sets~\cite{Zaheer2017}. The count and pooled descriptors allow a single network to act on different particle cardinalities.

A shared particle--query decoder $\Psi_{\theta_{\full}}$ then produces one raw coefficient per pair:
\begin{equation}
 \widetilde R_{cqp}^{\full}
 =\Psi_{\theta_{\full}}\!\left(
 [\vct e_{cp}^{\full},\vct u_c^{\full},
    \vct\xi_q,\vct\xi_q-\vct\xi_{cp}]\right).
 \label{eq:decoder}
\end{equation}
Both encoder and decoder are multilayer perceptrons. The encoder input has dimension $d+1$, the pooled descriptor has dimension $2d_{\mathrm f}+1$, and the pair input has dimension $3d_{\mathrm f}+1+2d$. The output layer is linear, allowing signed coefficients. Particle stresses are applied only after these coefficients have been constructed; they do not enter the geometric feature path.

Variable-size particle sets are stored in arrays of capacity $P_{\max}$, together with a binary mask $\chi_{cp}$ that is one for a valid particle and zero for an unused slot. Invalid slots are excluded from the features, pooling, coefficient projection, and stress application. In padded-array expressions, the members of $\mathcal P_c$ are enumerated by local slots; this relabeling does not change their particle identities. Padding is a storage convention rather than an augmentation of the physical particle set. Permuting valid particles permutes the coefficient columns and the corresponding input stresses together, leaving the reconstructed stress unchanged up to floating-point summation effects.

\subsubsection{Constant projection and affine consistency}
\label{sec:constraints}

The raw decoder output has no automatic reproduction property. A spatially constant tensor $\stress_0$ is reconstructed exactly if and only if every coefficient row sums to one. We enforce this condition through a minimum Euclidean correction. Let $\widetilde{\vct r}_{cq}$ collect the valid raw coefficients at query $q$, and let $\vct 1$ be the vector of $P_c$ ones. The projected row is defined by
\begin{equation}
 \vct r_{cq}
 =\argmin_{\vct r}\frac12\norm{\vct r-\widetilde{\vct r}_{cq}}_2^2
 \quad\text{subject to}\quad \vct 1^{\T}\vct r=1.
 \label{eq:projectionproblem}
\end{equation}
The stationarity condition for a scalar multiplier $\lambda$ is $\vct r-\widetilde{\vct r}_{cq}+\lambda\vct1=0$. Eliminating $\lambda$ yields the explicit masked formula
\begin{equation}
 R_{cqp}^{\full}
 =\chi_{cp}\left[\widetilde R_{cqp}^{\full}
   +\frac{1-\sum_{r=1}^{P_{\max}}\chi_{cr}\widetilde R_{cqr}^{\full}}{P_c}\right],
 \qquad P_c=\sum_{p=1}^{P_{\max}}\chi_{cp}>0.
 \label{eq:projection}
\end{equation}
No iterative solve or coordinate-moment inversion is required. Since $\sum_pR_{cqp}^{\full}=1$, substituting $\stress_p=\stress_0$ into Eq.~\eqref{eq:genericreconstruction} gives $\widehat\stress_{cq}^{\full}=\stress_0$. The property holds for every geometry with at least one valid particle and preserves tensor symmetry because a scalar coefficient is shared by all components.

To assess affine reproduction, define the coordinate-moment defect at each query by
\begin{equation}
 \vct\delta_{cq}^{\full}
 :=\sum_{p\in\mathcal P_c}R_{cqp}^{\full}\vct\xi_{cp}-\vct\xi_q.
 \label{eq:affinedefect}
\end{equation}
Exact affine reproduction requires $\vct\delta_{cq}^{\full}=\vct0$ at every query. Rather than enforce this additional condition through a hard projection, we penalize its residual during training. Its physical meaning follows by taking an affine scalar stress component $\sigma_{\mathrm a}(\vct x)=\sigma_0+\vct b_\sigma\cdot(\vct x-\vct x_c)$, where $\vct b_\sigma$ is a constant stress gradient. The exact constant projection gives
\begin{equation}
 \widehat\sigma_{\mathrm a,cq}^{\full}
      -\sigma_{\mathrm a}(\vct x_{cq})
 =\frac h2\vct b_\sigma\cdot\vct\delta_{cq}^{\full}.
 \label{eq:affineidentity}
\end{equation}
The coordinate penalty therefore controls a specific contribution to reconstruction error, not an abstract measure of smoothness. A hard affine projection would require a particle cloud of sufficient affine rank and can become ill-conditioned near degenerate configurations. More fundamentally, arbitrary affine fields cannot be identified from too few independent samples. The constant-hard, affine-soft formulation remains well defined even for such sparse particle sets.

\Needspace{13\baselineskip}
\subsubsection{Internal-force reconstruction and error decomposition}
\label{sec:fullerror}

With the query rule and projected coefficients now specified, the full-cell reconstruction is completed by applying the operator to the particle stresses and integrating the result against the background-basis gradients:
\begin{equation}
 \begin{aligned}
 \widehat\stress_{cq}^{\full}
  &=\sum_{p\in\mathcal P_c}R_{cqp}^{\full}\stress_p,\\
 \widehat{\vct f}_{ic}^{\full}
  &=-\sum_{q=1}^{Q_{\full}}W_{cq}\widehat\stress_{cq}^{\full}
                                      \nabla N_i(\vct x_{cq}).
 \end{aligned}
 \label{eq:fullforce}
\end{equation}
Here $\mat R_c^{\full}$ has $Q_{\full}$ rows and $P_c$ valid columns, and the second line is evaluated for every $i\in\mathcal I_c$. The same reconstructed stress is used for all active nodes. The particle volumes influence the geometric input, whereas the physical measure of integration is supplied by $W_{cq}$; no additional factor $V_p$ multiplies the reconstructed stress. This closes the construction introduced in Section~\ref{sec:objective}: the network supplies a constrained stress-transfer operator, and the prescribed rule converts its output into a cell contribution to the internal force.

To distinguish the accuracy of these two operations, consider a common reference stress field $\stress$ at the current configuration. For any region $D\subseteq K_c$, write $\vct f_{ic}(D;\stress)=-\int_D\stress\nabla N_i\dd v$ for its exact contribution. The force $\vct f_{ic}^{\Gauss,\full}[\stress]$ in Eq.~\eqref{eq:gausstarget} instead uses exact samples of this field at the prescribed full-cell queries. Adding and subtracting that intermediate force gives
\begin{equation}
 \begin{aligned}
 \widehat{\vct f}_{ic}^{\full}-\vct f_{ic}(K_c;\stress)
 ={}&\underbrace{\bigl[\widehat{\vct f}_{ic}^{\full}
               -\vct f_{ic}^{\Gauss,\full}[\stress]\bigr]}_{\text{reconstruction error}}\\
 &+\underbrace{\bigl[\vct f_{ic}^{\Gauss,\full}[\stress]
               -\vct f_{ic}(K_c;\stress)\bigr]}_{\text{quadrature error}}.
 \end{aligned}
 \label{eq:fullerror}
\end{equation}
The first bracket measures the effect of replacing exact query stresses by reconstructed ones while keeping the rule fixed. It includes both the approximation made by the reconstruction and any error already present in the particle stresses. The second bracket measures the error of that rule when supplied with exact stresses, and may remain nonzero even when reconstruction is perfect. There is no geometric term for a genuinely full cell because its material region is exactly $K_c$. In particular, the assumption here is full material occupancy, not merely the absence of a boundary label in a numerical classification.

The affine defect explains part of the first bracket. Define $\Lambda_c^{\full}=\max_q\sum_p\abs{R_{cqp}^{\full}}$ and $\delta_c^{\full}=\max_q\norm{\vct\delta_{cq}^{\full}}_2$. Suppose a reference stress field is twice continuously differentiable on the segments joining queries to particles, with first- and second-derivative bounds $M_{\sigma,1,c}$ and $M_{\sigma,2,c}$ in induced tensor norms. Using the tensor Frobenius norm $\norm{\mat A}_{\Frob}^2=\sum_{a,b}A_{ab}^2$, suppose that particle-stress perturbations have norm at most $\eta_c$. Taylor expansion then gives
\begin{equation}
 \max_q\norm{\widehat\stress_{cq}^{\full}-\stress(\vct x_{cq})}_{\Frob}
 \le \Lambda_c^{\full}\eta_c
   +\frac h2M_{\sigma,1,c}\delta_c^{\full}
   +\frac{d h^2}{2}M_{\sigma,2,c}\Lambda_c^{\full}.
 \label{eq:reconstructionbound}
\end{equation}
\ref{app:error} derives this estimate and the weighted force bound in Eq.~\eqref{eq:weightedforcebound}, which transfers the stress error to the first bracket of Eq.~\eqref{eq:fullerror}. The three contributions in Eq.~\eqref{eq:reconstructionbound} are amplified particle error, the affine-moment defect, and unresolved stress curvature. A unit row sum alone supplies no upper bound on $\Lambda_c^{\full}$, and the soft penalty does not by itself establish a convergence rate. These are analytical measures of the reconstructed operator, rather than quantities used by an online error controller. They also leave the quadrature bracket unchanged: increasing reconstruction accuracy and increasing quadrature order address different parts of the total force error.

The full-cell construction thus separates an assumed exact integration region, a prescribed quadrature rule, and a learned stress-transfer operator. A cut cell retains this separation, but the integration region must first be represented inside the parent span. The next section follows the same construction and shows where that additional geometric approximation enters the force error.


==> sections/24_cut.tex <==
\subsection{Extension to cut cells in a dimension-independent form}
\label{sec:cut}

\subsubsection{Reconstruction domain and prescribed quadrature}

The full-cell construction assumes that the integration region is all of $K_c$. When a material boundary intersects that cell, the correct domain is instead $D_c=\Omega(t)\cap K_c$. Extending the full-cell rule into the empty part of the cell would introduce a geometric integration error, irrespective of the accuracy of the reconstructed stress. The cut-cell extension therefore retains the parent-cell basis and particle set, but places its quadrature points inside an approximation of the material region.

A locally planar boundary is represented by a unit normal $\vct n_c$ directed into the material and a signed offset $\kappa_c$ from the parent center. The reconstructed material region is
\begin{equation}
 D_c^{\mathrm{rec}}
 =K_c\cap\{\vct x:\vct n_c\cdot(\vct x-\vct x_c)-\kappa_c\ge0\},
 \qquad
 \alpha_c=\frac{\abs{D_c^{\mathrm{rec}}}}{\abs{K_c}}.
 \label{eq:cutgeometry}
\end{equation}
Here $\alpha_c\in(0,1)$ is the material fraction. The superscript $\mathrm{rec}$ distinguishes the represented geometry from the exact intersection $D_c$; they coincide only when the local boundary model is exact. Particle positions and supplied boundary labels determine whether such a local representation is admissible in the solver. The reconstruction formulation uses the resulting region and does not require a particular line- or plane-fitting algorithm.

Partition the represented region into $N_{\simp,c}$ nonoverlapping $d$-simplices $T_{c\ell}$, with child index $\ell=1,\ldots,N_{\simp,c}$:
\begin{equation}
 \overline{D_c^{\mathrm{rec}}}
 =\bigcup_{\ell=1}^{N_{\simp,c}}\overline{T_{c\ell}},
 \qquad
 \abs{T_{c\ell}\cap T_{cm}}=0\quad(\ell\ne m).
 \label{eq:simplexpartition}
\end{equation}
Let $\widehat T=\{\vct\eta\in\R^d:\eta_a\ge0,\ \sum_a\eta_a\le1\}$ be the reference simplex. For the vertices $\vct x_{c\ell}^{(0)},\ldots,\vct x_{c\ell}^{(d)}$, define the edge matrix $\mat A_{c\ell}=[\vct x_{c\ell}^{(1)}-\vct x_{c\ell}^{(0)},\ldots,\vct x_{c\ell}^{(d)}-\vct x_{c\ell}^{(0)}]$. A rule with $Q_{\simp}$ reference points $\vct\eta_q$ and positive reference weights $\widehat\omega_q$ gives
\begin{equation}
 \begin{aligned}
 \vct x_{c\ell q}&=\vct x_{c\ell}^{(0)}+\mat A_{c\ell}\vct\eta_q,\\
 W_{c\ell q}&=\abs{\det\mat A_{c\ell}}\widehat\omega_q,
 &\vct\xi_{c\ell q}&=\frac2h(\vct x_{c\ell q}-\vct x_c).
 \end{aligned}
 \label{eq:simplexrule}
\end{equation}
The rule is chosen to integrate constants exactly, so $\sum_qW_{c\ell q}=\abs{T_{c\ell}}$. The complete parent has $Q_{\cut}(c)=N_{\simp,c}Q_{\simp}$ query points and $\sum_{\ell,q}W_{c\ell q}=\abs{D_c^{\mathrm{rec}}}$. The two indices $\ell,q$ are retained to distinguish a simplex-local rule from its parent-cell assembly. A tensor-product Duffy construction~\cite{Duffy1982}, including its dimension-dependent Jacobian, is given in \ref{app:quadrature}.

Although a simplex map is used to generate the integration points, the neural coordinates $\vct\xi_{c\ell q}$ remain coordinates in the parent span. Background gradients are likewise evaluated from the parent basis, not from simplex finite element functions. The simplices partition the integration region; they do not create new mechanical degrees of freedom or replace the background interpolation.

\subsubsection{Geometry-conditioned reconstruction coefficients}

For every simplex, the network uses the complete parent set $\mathcal P_c$, rather than only particles lying inside $T_{c\ell}$. Each child operator $\mat R_{c\ell}^{\cut}$ therefore has $Q_{\simp}$ query rows and $P_c$ valid particle columns. As in the full-cell module, its coefficients are constructed from geometry before being applied to stress. The additional child index identifies the subregion containing the queries; it does not change which particles supply the material state.

The cut volume feature is formed from the model input volume $V_{cp}^{\mathrm{in}}$ and the associated material-volume scale $V_c^{\mathrm{scale}}$. Together with the parent-local particle position, it defines
\begin{equation}
 \nu_{cp}^{\cut}=V_{cp}^{\mathrm{in}}/V_c^{\mathrm{scale}},
 \qquad
 \vct z_{cp}^{\cut}=[\vct\xi_{cp},\nu_{cp}^{\cut}].
 \label{eq:cutvolfeature}
\end{equation}
In cut-cell training, these are the particle volume and the complete represented material volume, respectively, not the individual simplex volume. An online adapter must express both in the coordinate and normalization convention of its model. As for the full-cell input, this operation does not modify physical particle volumes or integration weights.

The shared particle encoder $\Phi_{\theta_{\cut}}$ and pooled parent descriptor use the same construction as in Eq.~\eqref{eq:pooling}, with a separately trained parameter set $\theta_{\cut}$:
\begin{equation}
 \begin{aligned}
 \vct e_{cp}^{\cut}&=\Phi_{\theta_{\cut}}(\vct z_{cp}^{\cut}),\\
 \vct u_c^{\cut}&=\left[
  \frac1{P_c}\sum_p\vct e_{cp}^{\cut},\quad
  \sum_p\vct e_{cp}^{\cut},\quad P_c/P_{\max}\right].
 \end{aligned}
 \label{eq:cutpooling}
\end{equation}
These features describe the whole parent and are shared by its children. To identify the queried subregion, a context encoder $\mathcal U_{\theta_{\cut}}$ embeds a geometric descriptor $\vct c_{c\ell}$ into a feature $\vct e_{c\ell}^{\mathrm{ctx}}$. The descriptor contains dimensionless measures and centroids of the simplex and material region, the oriented boundary plane, and the fixed child-order information used by the model. The raw coefficients are
\begin{equation}
 \begin{aligned}
 \vct e_{c\ell}^{\mathrm{ctx}}&=\mathcal U_{\theta_{\cut}}(\vct c_{c\ell}),\\
 \widetilde R_{c\ell qp}^{\cut}
  &=\Psi_{\theta_{\cut}}\!\left(
  [\vct e_{cp}^{\cut},\vct u_c^{\cut},\vct e_{c\ell}^{\mathrm{ctx}},
   \vct\xi_{c\ell q},\vct\xi_{c\ell q}-\vct\xi_{cp}]\right).
 \end{aligned}
 \label{eq:cutdecoder}
\end{equation}
\ref{app:context} gives an explicit descriptor and its dimensional specialization. Including child-order information makes a consistent decomposition and ordering part of the model interface; particle-permutation invariance should not be confused with invariance to an arbitrary retriangulation or retessellation.

\subsubsection{Constant projection and affine consistency}

The minimum-correction problem in Eq.~\eqref{eq:projectionproblem} is applied independently to every child-query row. With the parent mask and particle count, it gives
\begin{equation}
 \begin{aligned}
 R_{c\ell qp}^{\cut}
 &=\chi_{cp}\left[\widetilde R_{c\ell qp}^{\cut}
 +\frac{1-\sum_{r=1}^{P_{\max}}\chi_{cr}\widetilde R_{c\ell qr}^{\cut}}{P_c}\right],\\
 \vct\delta_{c\ell q}^{\cut}
 &=\sum_{p\in\mathcal P_c}R_{c\ell qp}^{\cut}\vct\xi_{cp}
                                      -\vct\xi_{c\ell q}.
 \end{aligned}
 \label{eq:cutconstraints}
\end{equation}
The row sum is one at every query, so constant stress is reproduced on every simplex. Exact affine reproduction would additionally require $\vct\delta_{c\ell q}^{\cut}=\vct0$, which is again treated as a soft condition. Because particles and queries use the same parent coordinates, the affine scalar field and gradient $\vct b_\sigma$ introduced in Section~\ref{sec:constraints} satisfy the direct counterpart of Eq.~\eqref{eq:affineidentity}:
\begin{equation}
 \widehat\sigma_{\mathrm a,c\ell q}^{\cut}
      -\sigma_{\mathrm a}(\vct x_{c\ell q})
 =\frac h2\vct b_\sigma\cdot\vct\delta_{c\ell q}^{\cut}.
 \label{eq:cutaffineidentity}
\end{equation}
The soft residual consequently has the same physical meaning in both modules. For $P_c=1$, the valid coefficient must be one at every query, so the only possible prediction is the single particle stress. This limiting case makes the information content of the method explicit and explains why sparse cut cells require separate evaluation.

\Needspace{13\baselineskip}
\subsubsection{Internal-force reconstruction and error decomposition}
\label{sec:cuterror}

Applying the projected child operators to the particle stresses completes the cut-cell reconstruction. The resulting stresses are integrated first over each simplex and then summed over the parent:
\begin{equation}
 \begin{aligned}
 \widehat\stress_{c\ell q}^{\cut}
  &=\sum_{p\in\mathcal P_c}R_{c\ell qp}^{\cut}\stress_p,\\
 \widehat{\vct f}_{ic}^{\cut}
  &=-\sum_{\ell=1}^{N_{\simp,c}}\sum_{q=1}^{Q_{\simp}}
          W_{c\ell q}\widehat\stress_{c\ell q}^{\cut}
                              \nabla N_i(\vct x_{c\ell q}).
 \end{aligned}
 \label{eq:cutforce}
\end{equation}
The two lines have the same roles as in Eq.~\eqref{eq:fullforce}; only the query indexing and the integration region change. Every child uses the parent basis $N_i$ and contributes to the same active-node set $\mathcal I_c$. A simplex with no particle in its own interior can still be reconstructed from the parent data. Reusing those data does not duplicate material volume, because the physical weights belong to disjoint integration regions and each child is included exactly once.

As for the full cell, introduce the intermediate force obtained by supplying exact reference stresses to the same quadrature rule:
\begin{equation}
 \vct f_{ic}^{\Gauss,\cut}[\stress]
 =-\sum_{\ell=1}^{N_{\simp,c}}\sum_{q=1}^{Q_{\simp}}
  W_{c\ell q}\stress(\vct x_{c\ell q})\nabla N_i(\vct x_{c\ell q}).
 \label{eq:cutgausstarget}
\end{equation}
This is the counterpart of Eq.~\eqref{eq:gausstarget}, now on $D_c^{\mathrm{rec}}$. Using the exact-region force $\vct f_{ic}(D;\stress)$ defined in Section~\ref{sec:fullerror}, add and subtract both this quadrature force and the exact integral over the represented region. The full-cell decomposition then extends to
\begin{equation}
 \begin{aligned}
 \widehat{\vct f}_{ic}^{\cut}-\vct f_{ic}(D_c;\stress)
 ={}&\underbrace{\bigl[\widehat{\vct f}_{ic}^{\cut}
               -\vct f_{ic}^{\Gauss,\cut}[\stress]\bigr]}_{\text{reconstruction error}}\\
 &+\underbrace{\bigl[\vct f_{ic}^{\Gauss,\cut}[\stress]
               -\vct f_{ic}(D_c^{\mathrm{rec}};\stress)\bigr]}_{\text{quadrature error}}\\
 &+\underbrace{\bigl[\vct f_{ic}(D_c^{\mathrm{rec}};\stress)
               -\vct f_{ic}(D_c;\stress)\bigr]}_{\text{geometry error}}.
 \end{aligned}
 \label{eq:cuterror}
\end{equation}
The first two brackets have precisely the meanings established in Eq.~\eqref{eq:fullerror}: stress reconstruction is assessed with the geometry and rule held fixed, and quadrature is assessed with exact query stresses on that same geometry. The third bracket is the additional effect of representing the material boundary. It vanishes when $D_c^{\mathrm{rec}}=D_c$, even though the parent may still be only partially occupied. Taking the represented and exact regions to be $K_c$ recovers the two-term full-cell error structure. This reduction concerns the error structure; each module retains its own prescribed rule and trained operator.

The reconstruction term is controlled by the same local estimate as in the full-cell case. Define $\Lambda_c^{\cut}=\max_{\ell,q}\sum_p\abs{R_{c\ell qp}^{\cut}}$ and $\delta_c^{\cut}=\max_{\ell,q}\norm{\vct\delta_{c\ell q}^{\cut}}_2$. Under the same smoothness and particle-error assumptions as in Eq.~\eqref{eq:reconstructionbound}, with derivative bounds taken over all relevant particle--query segments, one obtains
\begin{equation}
 \max_{\ell,q}\norm{\widehat\stress_{c\ell q}^{\cut}-\stress(\vct x_{c\ell q})}_{\Frob}
 \le\Lambda_c^{\cut}\eta_c
  +\frac h2M_{\sigma,1,c}\delta_c^{\cut}
  +\frac{d h^2}{2}M_{\sigma,2,c}\Lambda_c^{\cut}.
 \label{eq:cutreconstructionbound}
\end{equation}
The length scale remains the parent spacing $h$, rather than an individual simplex diameter, because every child uses particles from throughout the parent. The weighted force bound in \ref{app:error} likewise applies with the complete $\ell,q$ sum. These estimates concern the first bracket only; quadrature order controls a different approximation, and the geometric discrepancy is bounded separately by Eq.~\eqref{eq:geometrybound}. The parallel decompositions therefore provide a common basis for evaluating both modules, while identifying boundary representation as the additional source of error in a cut cell.


==> sections/25_data.tex <==
\subsection{Analytical training fields and data construction}
\label{sec:data}

\subsubsection{Independent geometries and stress realizations}

The reconstruction is trained offline so that its target can be evaluated independently of a complete MPM simulation. Each sample comprises a particle geometry, one prescribed integration rule, and analytical stress fields evaluated both at the particles and at that rule's queries. This construction isolates the quality of the particle-to-quadrature transfer from errors in the constitutive update, time integration, loading, and boundary enforcement. A geometry is indexed by $c$ and its stress realizations by $s=1,\ldots,S$. Superscript $*$ denotes an analytical stress field; superscript $\Gauss$ continues to denote its discrete force obtained with the selected quadrature.

For a full-cell realization, the labels and predictions are
\begin{equation}
 \begin{aligned}
 \stress_{csp}^{*}&=\stress_{cs}^{*}(\vct x_p),
 &\stress_{csq}^{*}&=\stress_{cs}^{*}(\vct x_{cq}),\\
 \widehat\stress_{csq}^{\full}
  &=\sum_{p\in\mathcal P_c}R_{cqp}^{\full}\stress_{csp}^{*},
 &\vct f_{ics}^{\Gauss,\full}
  &=-\sum_{q=1}^{Q_{\full}}W_{cq}\stress_{csq}^{*}
                                       \nabla N_i(\vct x_{cq}).
 \end{aligned}
 \label{eq:fulllabels}
\end{equation}
The predicted force $\widehat{\vct f}_{ics}^{\full}$ uses the same weights and gradients with $\widehat\stress_{csq}^{\full}$ in place of $\stress_{csq}^{*}$. In a cut cell, query labels carry the additional child index, $\stress_{cs\ell q}^{*}=\stress_{cs}^{*}(\vct x_{c\ell q})$, and both predicted and reference forces are assembled over all children before they enter the parent objective. Every realization of one geometry uses the same reconstruction matrices; the network cannot adapt its coefficients to the particular stress values of that realization.

\subsubsection{Analytical field families}
\label{sec:fields}

The training fields comprise constant, linear, quadratic, and trigonometric variations in the parent coordinates. They supply different spatial content while keeping their values available analytically at arbitrary particle and query locations. To display their definitions without repetitive geometry and realization subscripts, consider one unscaled field $\widetilde\stress(\vct\xi)$. The tensors $\mat\Sigma_0$, $\mat\Sigma_a$, and $\mat\Sigma_{ab}$ below are independently sampled symmetric coefficient tensors, not stresses obtained from a boundary-value solution. The polynomial families are
\begin{align}
 \widetilde\stress^{\mathrm{constant}}(\vct\xi)
    &=\mat\Sigma_0,
    \label{eq:fieldconstant}\\
 \widetilde\stress^{\mathrm{linear}}(\vct\xi)
    &=\mat\Sigma_0+\sum_{a=1}^{d}\mat\Sigma_a\xi_a,
    \label{eq:fieldlinear}\\
 \widetilde\stress^{\mathrm{quadratic}}(\vct\xi)
    &=\mat\Sigma_0+\sum_{a=1}^{d}\mat\Sigma_a\xi_a
      +\sum_{1\le a\le b\le d}\mat\Sigma_{ab}\xi_a\xi_b.
    \label{eq:fieldquadratic}
\end{align}
The quadratic family spans all monomials of total degree at most two. In particular, the mixed term is retained rather than replacing the field by a sum of one-dimensional quadratics. The independent coefficients for the diagonal and off-diagonal components allow normal and shear variations to be sampled independently, while each coefficient tensor is mirrored across its diagonal to enforce symmetry.

A dimension-independent notation for the trigonometric family is
\begin{equation}
 \begin{aligned}
 \widetilde\stress^{\mathrm{trig}}(\vct\xi)
  ={}&\mat\Sigma_0
  +\sum_{a=1}^{d}\left[
     \mat\Sigma_a^{\sin}\sin(\pi\xi_a)
    +\mat\Sigma_a^{\cos}\cos(\pi\xi_a)\right]\\
  &+\sum_{(a,b)\in\mathcal E_d}
       \mat\Sigma_{ab}^{\mathrm{mix}}
          \sin(\pi\xi_a)\cos(\pi\xi_b),
 \end{aligned}
 \label{eq:fieldtrig}
\end{equation}
where $\mathcal E_d$ specifies the ordered coordinate pairs included as mixed modes. The mode list is part of the analytical data definition. In the two-dimensional bank, $\mathcal E_2=\{(1,2)\}$, so the scalar basis is explicitly
\begin{equation}
 \vct b_{\mathrm{trig},2}(\xi_1,\xi_2)
 =\begin{bmatrix}
 1\\ \sin(\pi\xi_1)\\ \cos(\pi\xi_1)\\
 \sin(\pi\xi_2)\\ \cos(\pi\xi_2)\\
 \sin(\pi\xi_1)\cos(\pi\xi_2)
 \end{bmatrix}.
 \label{eq:trig2}
\end{equation}
The final mode couples the two coordinates and complements the separate axial variations. Dimensional extensions of Eq.~\eqref{eq:fieldtrig} also require their mixed-mode list to be retained with the dataset; a choice of three-dimensional modes is not implied by the two-dimensional list.

For the two-dimensional full-cell bank, each independent tensor component has independent standard-normal coefficients. A common scalar rescales the entire tensor field, preserving the relative normal and shear amplitudes. Let $\mathcal X_{\mathrm{norm}}$ be the $11\times11$ uniform grid on $[-1,1]^2$, let $\sigma_{\mathrm{amp}}>0$ be the target amplitude, and restore the indices $c,s$. The normalized field is
\begin{equation}
 \stress_{cs}^{*}(\vct x_c+(h/2)\vct\xi)
  =\gamma_{cs}\widetilde\stress_{cs}(\vct\xi),
 \qquad
 \gamma_{cs}
  =\frac{\sigma_{\mathrm{amp}}}
  {\displaystyle\max_{\vct\xi\in\mathcal X_{\mathrm{norm}}}
       \norm{\widetilde\stress_{cs}(\vct\xi)}_{\Frob}}.
 \label{eq:fieldnormalization}
\end{equation}
The Frobenius norm is $\norm{\mat A}_{\Frob}^2=\sum_{a,b}A_{ab}^2$, so an off-diagonal component is counted twice. Numerically vanishing realizations are resampled. The polynomial and trigonometric coefficients and $\gamma_{cs}$ are stored, allowing evaluation at any later quadrature order without interpolating existing labels. This amplitude scaling is an offline data convention; the online operator acts directly on physical particle stresses.

These fields need not satisfy equilibrium with one common body force or boundary traction. Their purpose is to probe a local linear integration map using exactly known spatial variation. The constant family tests the imposed reproduction condition, the linear family exposes coordinate-moment defects, the quadratic family probes curvature, and the trigonometric family provides smooth nonpolynomial variation. Gaussian stress profiles are not included in the formal four-family bank.

\subsubsection{Particle configurations, model scopes, and held-out sets}
\label{sec:datasets}

The numerical study evaluates two-dimensional full- and cut-cell models and three-dimensional full-cell models. Table~\ref{tab:scope} separates these implemented scopes from the dimension-independent formulation. In two dimensions the integration children are triangles. No three-dimensional cut-cell result or unstructured-mesh result is implied by the general equations in Sections~\ref{sec:objective}--\ref{sec:cut}.

\begin{table}[htbp]
\centering\small
\caption{Model families and particle-count envelopes in the study. G$g$ denotes a one-dimensional tensor-product order, not a total point count or an exactness degree. A separate model is associated with each basis--rule pair.}
\label{tab:scope}
\begin{tabularx}{\textwidth}{@{}lYYY@{}}
\toprule
Quantity & 2D full cell & 2D cut cell & 3D full cell\\
\midrule
Basis degree $k$ & $1,2,3$ & $1,2,3$ & $1,2,3$\\
Particle count $P_c$ & Every integer $4$--$36$ & Every integer $1$--$36$ per parent & Every integer $4$--$36$\\
Rule choices & G4, G6 & G2, G3 per triangle & G2, G3\\
Queries & $Q_{\full}=16,36$ & $Q_{\simp}=4,9$ per triangle & $Q_{\full}=8,27$\\
Active parent nodes & $(k+1)^2$ & $(k+1)^2$ & $(k+1)^3$\\
State component order & $11,22,12$ & $11,22,12$ & $11,22,33,$\newline $12,13,23$\\
\bottomrule
\end{tabularx}
\end{table}

The full-cell geometries are balanced by the actual number of particles, not by a particles-per-axis parameter. The two-dimensional profile has 500 geometries at each of the 33 counts from 4 to 36. It combines five layout families with the proportions in Table~\ref{tab:layouts}. Stratified samples provide broadly distributed coverage, random gaps vary local occupancy, affine distortions alter alignment, clustered samples concentrate coverage, and boundary-crossing layouts mimic changed occupancy after transport. The last name describes a particle-placement pattern in a full material cell; it is not a cut-cell geometry.

\begin{table}[htbp]
\centering\small
\caption{Two-dimensional full-cell geometry mixture. Counts are per particle cardinality in the 500-geometry profile.}
\label{tab:layouts}
\begin{tabularx}{\textwidth}{@{}lrrY@{}}
\toprule
Layout & Fraction & Count & Geometric variation\\
\midrule
Stratified & $0.45$ & 225 & Quasi-uniform, coverage-preserving placement\\
Random gap & $0.15$ & 75 & Removal from an oversampled candidate set\\
Affine deformed & $0.15$ & 75 & Bounded stretching and shear\\
Clustered & $0.15$ & 75 & Correlated contraction and displacement\\
Boundary crossing & $0.10$ & 50 & Shifted occupancy with periodic wrapping\\
\bottomrule
\end{tabularx}
\end{table}

The position jitter is 0.30 of the local sampling-stratum width, while additional volume and particle-domain descriptor jitter are both zero. Thus the full-cell training volumes satisfy $V_p=\abs{K_c}/P_c$. The network remains capable of receiving relative-volume features, but the absence of volume jitter must not be interpreted as training over arbitrary volume distributions. The bounded layout parameters are given in \ref{app:layoutparameters} so that the distribution is reproducible without interrupting the formulation.

Each full-cell geometry is paired with 12 stress realizations, three from each family. The split is made by geometry and stratified by $P_c$, giving the counts in Table~\ref{tab:datacounts}. All realizations of one geometry remain in the same subset. The same rule applies to a cut parent: all of its simplices and all attached stresses belong to one subset. Otherwise a test realization could reuse a particle cloud or a parent geometry already observed in training, despite having different stress coefficients.

\begin{table}[htbp]
\centering\small
\caption{Two-dimensional full-cell data and evaluation profile. Counts are per basis--rule dataset; the shared geometry/field bank prevents basis and order comparisons from being confounded by different samples.}
\label{tab:datacounts}
\begin{tabularx}{\textwidth}{@{}lY@{}}
\toprule
Parameter & Specification\\
\midrule
Reference parent & Unit square; neural coordinates in $[-1,1]^2$\\
Geometries & $33\times500=16{,}500$\\
Realizations per geometry & $S=12$; three per analytical family\\
Total geometry--stress pairs & $198{,}000$\\
Training / validation / test & $80\%/10\%/10\%$ by geometry\\
Geometries per count and split & $400/50/50$\\
Total geometries per split & $13{,}200/1{,}650/1{,}650$\\
Stress pairs per split & $158{,}400/19{,}800/19{,}800$\\
Amplitude / coefficient sampling & $\sigma_{\mathrm{amp}}=1$; independent normal coefficients\\
Position / volume / domain jitter & $0.30/0/0$\\
Geometry-bank seed & 2026\\
Nominal model-training seed & 2027; each run retains its own seed\\
Arithmetic & Double precision\\
\bottomrule
\end{tabularx}
\end{table}

Paired comparisons across basis families and full-cell Gauss orders use matching particle geometries, field coefficients, and splits. The cut-cell bank additionally varies its represented material fraction and interface orientation, and includes the sparse parent counts $P_c=1,2,3$ rather than excluding them through a simplex-local particle requirement. Dataset sizes and sampling ranges are module-specific: the counts in Table~\ref{tab:datacounts} specify the two-dimensional full-cell profile and are not transferred to the cut or three-dimensional banks by assumption. In all cases, the saved geometry, field coefficients, and split identities define the samples used for training and independent evaluation.


==> sections/26_training.tex <==
\subsection{Learning objectives, optimization, and evaluation}
\label{sec:losses}

\subsubsection{Full-cell objective}

The objectives now make the force-oriented choice of Section~\ref{sec:forcechoice} concrete. Let $\vct s_{csq}^{*}=\operatorname{sv}(\stress_{csq}^{*})$ and $\widehat{\vct s}_{csq}^{\full}=\operatorname{sv}(\widehat\stress_{csq}^{\full})$. Stack the nodal forces for realization $s$ into $\vct f_{cs}^{\Gauss,\full}$ and $\widehat{\vct f}_{cs}^{\full}$, using the node and component order defined in Eq.~\eqref{eq:forceoperator}. Their dimension is $dN_{b,c}$. The stress-component norm below counts an off-diagonal component once; it therefore differs from the tensor Frobenius norm used in Eq.~\eqref{eq:fieldnormalization}.

Let $\varsigma_{cs}$ be the root-mean-square scale of the query stress, floored by a positive training-set scale $\varsigma_{\min}$:
\begin{equation}
 \varsigma_{cs}^{2}
 =\max\left\{\frac1{n_\sigma Q_{\full}}
       \sum_{q=1}^{Q_{\full}}\norm{\vct s_{csq}^{*}}_2^2,
       \varsigma_{\min}^{2}\right\}.
 \label{eq:stressscale}
\end{equation}
For the two-dimensional full-cell training profile, the characteristic force norm is $f_{cs}^{\mathrm{char}}=\sqrt{2N_{b,c}}\,h\varsigma_{cs}$, with units of force per unit thickness. More generally, the selected characteristic force scale is part of the model's normalization; its dimensionally consistent isotropic extension scales with $\varsigma_{cs}h^{d-1}$. Keeping this definition explicit prevents a two-dimensional area factor from being silently reused as a three-dimensional force scale.

With a fixed nonnegative dimensionless floor ratio $r_0$, the per-realization losses are
\begin{equation}
 \begin{aligned}
 L_{f,cs}^{\full}
 &=\frac{\norm{\widehat{\vct f}_{cs}^{\full}
                       -\vct f_{cs}^{\Gauss,\full}}_2}
 {\sqrt{\norm{\vct f_{cs}^{\Gauss,\full}}_2^2
                     +(r_0f_{cs}^{\mathrm{char}})^2}},\\
 L_{\sigma,cs}^{\full}
 &=\frac{\displaystyle\sum_{q=1}^{Q_{\full}}
           \norm{\widehat{\vct s}_{csq}^{\full}-\vct s_{csq}^{*}}_2^2}
          {n_\sigma Q_{\full}\varsigma_{cs}^2},\\
 L_{\mathrm{lin},c}^{\full}
 &=\frac1{dQ_{\full}}\sum_{q=1}^{Q_{\full}}
                    \norm{\vct\delta_{cq}^{\full}}_2^2.
 \end{aligned}
 \label{eq:fulllosses}
\end{equation}
The force loss is an unsquared stabilized relative error. Its denominator is bounded below by the smallest positive representable value in the numerical implementation, including when an explicitly selected $r_0=0$ coincides with a vanishing target force. The stress loss is an unweighted mean squared error over query points and independent tensor components. Gauss weights enter the force assembly, but they are not inserted into this particular stress loss. The linear term is purely geometric and uses the coordinate defect already defined in Eq.~\eqref{eq:affinedefect}.

Let $\mathcal D_{\full}^{\mathrm{tr}}$ be the training geometry set and $N_{\full}^{\mathrm{tr}}$ its size. For equal numbers of stress realizations per geometry, the full-cell objective is
\begin{equation}
 \mathcal L_{\full}
 =\frac1{N_{\full}^{\mathrm{tr}}S}
   \sum_{c\in\mathcal D_{\full}^{\mathrm{tr}}}\sum_{s=1}^{S}
      \left[L_{f,cs}^{\full}
             +0.25L_{\sigma,cs}^{\full}
             +0.25L_{\mathrm{lin},c}^{\full}\right].
 \label{eq:fullobjective}
\end{equation}
Repeating the geometric term over $s$ does not change its relative geometry weighting because $S$ is constant. The constant condition requires no loss term: it is already imposed by Eq.~\eqref{eq:projection}. No reconstruction-coefficient norm penalty is active in this profile. AdamW weight decay, specified below, acts on network parameters and is a different operation.

Near-zero target forces are stabilized to prevent a few cases from dominating the objective solely through division by a very small norm. In the stated profile, $r_0$ is determined once as the fifth percentile of $\norm{\vct f_{cs}^{\Gauss,\full}}_2/f_{cs}^{\mathrm{char}}$ over the training subset. The stress floor is $10^{-8}$ times the training-set global component RMS. Neither quantity is recalibrated on validation or test data. A run with an explicitly prescribed force floor records that value instead of recalculating it from another subset.

\subsubsection{Cut-parent objective}
\label{sec:cutloss}

For a cut cell, the network is evaluated on individual simplices, but the force being approximated belongs to the complete material portion of the parent. Denote its stacked reference and predicted forces by $\vct f_{cs}^{\Gauss,\cut}$ and $\widehat{\vct f}_{cs}^{\cut}$, and its query component vectors by $\vct s_{cs\ell q}^{*}$ and $\widehat{\vct s}_{cs\ell q}^{\cut}$. The parent-aggregated loss formulation is
\begin{equation}
 \begin{aligned}
 L_{f,cs}^{\cut}
 &=\frac{\norm{\widehat{\vct f}_{cs}^{\cut}
                        -\vct f_{cs}^{\Gauss,\cut}}_2^2}
         {\norm{\vct f_{cs}^{\Gauss,\cut}}_2^2+\varepsilon_{f,\cut}},\\
 L_{\sigma,cs}^{\cut}
 &=\frac{\displaystyle\sum_{\ell=1}^{N_{\simp,c}}\sum_{q=1}^{Q_{\simp}}
       W_{c\ell q}\norm{\widehat{\vct s}_{cs\ell q}^{\cut}
                                     -\vct s_{cs\ell q}^{*}}_2^2}
       {\displaystyle\sum_{\ell=1}^{N_{\simp,c}}\sum_{q=1}^{Q_{\simp}}
       W_{c\ell q}\norm{\vct s_{cs\ell q}^{*}}_2^2+\varepsilon_{\sigma,\cut}},\\
 L_{\mathrm{lin},c}^{\cut}
 &=\frac1{dN_{\simp,c}Q_{\simp}}
       \sum_{\ell=1}^{N_{\simp,c}}\sum_{q=1}^{Q_{\simp}}
                       \norm{\vct\delta_{c\ell q}^{\cut}}_2^2.
 \end{aligned}
 \label{eq:cutlosses}
\end{equation}
The positive denominator floors $\varepsilon_{f,\cut}$ and $\varepsilon_{\sigma,\cut}$ have the units of their respective squared-force and integrated squared-stress denominators. A code using nondimensional training data may store the same numerical epsilon in both places; that does not make these two dimensional quantities identical.

This cut-cell force term is squared, unlike the full-cell force term, and its stress term is weighted by physical quadrature volume. The weights prevent a very small simplex from receiving the same stress-error influence as a large one merely because both have $Q_{\simp}$ queries. Most importantly, the simplex forces are added before computing $L_{f,cs}^{\cut}$. If $\vct e_{cs\ell}^{f}$ denotes the nodal-force error contributed by child $\ell$, then
\begin{equation}
 \norm{\sum_\ell\vct e_{cs\ell}^{f}}_2^2
 =\sum_\ell\norm{\vct e_{cs\ell}^{f}}_2^2
  +2\sum_{\ell<m}(\vct e_{cs\ell}^{f})^{\T}\vct e_{csm}^{f}.
 \label{eq:crosschild}
\end{equation}
Independently normalized child-force losses would omit these cross terms and optimize a different quantity from the parent force assembled in the solver. They would also give more training weight to parents partitioned into more children.

Let $\mathcal D_{\cut}^{\mathrm{tr}}$ contain $N_{\cut}^{\mathrm{tr}}$ cut parents. With module-specific coefficients $\lambda_{f,\cut}$, $\lambda_{\sigma,\cut}$, and $\lambda_{\mathrm{lin},\cut}$, the objective is
\begin{equation}
 \mathcal L_{\cut}
 =\frac1{N_{\cut}^{\mathrm{tr}}S}
   \sum_{c\in\mathcal D_{\cut}^{\mathrm{tr}}}\sum_{s=1}^{S}
      \left[\lambda_{f,\cut}L_{f,cs}^{\cut}
      +\lambda_{\sigma,\cut}L_{\sigma,cs}^{\cut}
      +\lambda_{\mathrm{lin},\cut}L_{\mathrm{lin},c}^{\cut}\right].
 \label{eq:cutobjective}
\end{equation}
The coefficients and denominator floors are retained as part of the cut model specification; the full-cell values in Eq.~\eqref{eq:fullobjective} are not substituted for them. The common methodological choice is force-oriented supervision with auxiliary stress and affine terms, not a requirement that the two modules use numerically identical objectives.

\subsubsection{Optimization and validation-based selection}
\label{sec:optimization}

The full-cell profile uses AdamW~\cite{Loshchilov2019}. In both modules, differentiation passes through the coefficient projection, stress reconstruction, and fixed force assembly, so the force objective directly updates the geometry-to-coefficient map. A batch comprises complete geometries and their attached stress realizations. For cut cells, valid simplices may be flattened into a computational batch for the neural forward pass, but they are reassembled to their parents before loss evaluation. This preserves the statistical unit of the data while permitting batched inference.

Table~\ref{tab:optimization} gives the canonical two-dimensional full-cell architecture and optimization parameters. Encoder and decoder weights are shared over particles and queries, respectively, and the SiLU activation is $\operatorname{SiLU}(z)=z/(1+\exp(-z))$. The cut model uses an additional context encoder, but its final model-specific settings are recorded separately. No inference-time fitting, optimizer step, or constitutive recalibration is performed in the MPM solver.

\begin{table}[htbp]
\centering\small
\caption{Canonical two-dimensional full-cell training and model-selection parameters. These settings describe the specified full-cell profile, not defaults presumed to apply to every cut-cell or three-dimensional checkpoint.}
\label{tab:optimization}
\begin{tabularx}{\textwidth}{@{}lY@{}}
\toprule
Parameter & Value or definition\\
\midrule
Feature width $d_{\mathrm f}$ & 64\\
Particle encoder / pair decoder & Three hidden layers each; SiLU; linear output\\
Optimizer & AdamW\\
Maximum epochs / batch size & 300 / 32 geometries\\
Initial / minimum learning rate & $10^{-3}$ / $10^{-6}$\\
Parameter weight decay & $10^{-6}$\\
Global gradient-norm clipping & 5\\
Learning-rate reduction & Factor $0.5$ after 10 plateau epochs\\
Scheduler monitor & Validation mean of $L_{f,cs}^{\full}$\\
Checkpoint and early-stopping monitor & Validation mean unsquared relative force error\\
Early-stopping patience & 30 epochs; minimum improvement $10^{-8}$\\
Force floor calibration & Training-only fifth percentile\\
Stress floor ratio & $10^{-8}$ of training-set component RMS\\
Reported relative-force epsilon & $10^{-14}$ in normalized data units\\
Precision & Float64 for data, model, and force assembly\\
\bottomrule
\end{tabularx}
\end{table}

Validation is used to select a checkpoint, not to update its parameters. The selection metric is the mean unsquared relative parent-force error on the validation set, both for full cells and for cut cells. It is distinct from the stabilized full-cell training objective and from the squared cut-cell objective. After selection, the chosen parameters are reloaded and evaluated on the untouched test set. Reporting test performance from this frozen checkpoint keeps test data out of optimization, learning-rate scheduling, early stopping, and model selection.

\subsubsection{Held-out errors and the quadrature target}
\label{sec:evaluation}

For a compact evaluation notation, let $M\in\{\full,\cut\}$ select a module, and let $\widehat{\vct f}_{cs}^{M}$ denote its complete cell or parent force. With a small reporting floor $\varepsilon_{\mathrm{rel},M}$ in force units, define
\begin{equation}
 e_{f,cs}^{\AI\to\Gauss,M}
  =\frac{\norm{\widehat{\vct f}_{cs}^{M}-\vct f_{cs}^{\Gauss,M}}_2}
         {\norm{\vct f_{cs}^{\Gauss,M}}_2+\varepsilon_{\mathrm{rel},M}},
 \qquad
 e_{f,cs}^{\MPM\to\Gauss,M}
  =\frac{\norm{\vct f_{cs}^{\MPM}-\vct f_{cs}^{\Gauss,M}}_2}
         {\norm{\vct f_{cs}^{\Gauss,M}}_2+\varepsilon_{\mathrm{rel},M}}.
 \label{eq:forceevaluation}
\end{equation}
The MPM force in this expression is computed from the same analytical particle stresses, positions, and volumes. Thus the comparison changes the integration operator without changing the available samples. A zero-force target should additionally be accompanied by an absolute or characteristic-scale error, because a relative ratio alone is not informative in that limit.

To measure stress recovery independently of force cancellation, let $\mathcal Q_c^{\full}=\{q:1\le q\le Q_{\full}\}$ and $\mathcal Q_c^{\cut}=\{(\ell,q):1\le\ell\le N_{\simp,c},\ 1\le q\le Q_{\simp}\}$. The dummy index $\mu$ denotes a member of the selected set, with the corresponding physical weight $W_{c\mu}$. A common physical-volume-weighted test metric is
\begin{equation}
 e_{\sigma,cs}^{M}
 =\frac{\left[\sum_{\mu\in\mathcal Q_c^M}W_{c\mu}
           \norm{\widehat{\vct s}_{cs\mu}^{M}-\vct s_{cs\mu}^{*}}_2^{2}
                         \right]^{1/2}}
        {\left[\sum_{\mu\in\mathcal Q_c^M}W_{c\mu}
           \norm{\vct s_{cs\mu}^{*}}_2^{2}\right]^{1/2}
                         +\varepsilon_{\mathrm{stress},M}}.
 \label{eq:stressevaluation}
\end{equation}
Here $\varepsilon_{\mathrm{stress},M}$ has stress-times-square-root-volume units. The component vectors use the same unscaled symmetric-tensor convention as the training losses. Volume weighting distinguishes this metric from the unweighted full-cell stress loss; counting each shear component once also distinguishes it from a tensor-Frobenius error. These choices are retained when comparing methods so that a change of norm is not mistaken for a change in reconstruction accuracy.

Analytical query values do not make a finite-order Gauss force an exact continuum reference. For this reason, a separate higher-order evaluation is constructed by resampling the stored analytical field, not by interpolating low-order query stresses. Let $\vct f_{cs}^{\mathrm{HO},M}$ be the resulting force on the same geometric domain. The evaluation distinguishes
\begin{equation}
 \underbrace{\widehat{\vct f}_{cs}^{M}-\vct f_{cs}^{\Gauss,M}}_{\text{reconstruction target error}},
 \qquad
 \underbrace{\vct f_{cs}^{\Gauss,M}-\vct f_{cs}^{\mathrm{HO},M}}_{\text{selected-rule discrepancy}},
 \qquad
 \underbrace{\widehat{\vct f}_{cs}^{M}-\vct f_{cs}^{\mathrm{HO},M}}_{\text{combined error}}.
 \label{eq:referencehierarchy}
\end{equation}
The corresponding MPM-to-HO error uses the same higher-order force. The full-cell evaluation profile uses G10 as the external higher-order comparator; adequacy is checked against successive orders, with polynomial cases also checked against the exactness conditions in \ref{app:quadrature}. For a cut cell, the same comparison leaves $D_c^{\mathrm{rec}}$ fixed, so it does not measure error in the reconstructed material boundary. Higher-order forces do not enter the training loss or checkpoint selection.

Test summaries are grouped by particle count and stress family and report the mean, median, upper percentiles, maximum, and fraction of paired cases in which AI-Q improves upon MPM. Layout- and material-fraction groups identify where coverage or geometry is influential. Each parent contributes once, irrespective of its number of simplices. The moment defects, coefficient amplification, and minimum particle coverage supplement the error statistics; they help distinguish inaccurate stress information from an inaccurate integration rule. Finally, timing uses fresh checkpoint inference and includes tensor preparation, geometric processing, network evaluation, and force assembly. Replaying saved predictions is useful for plotting, but is not a measurement of the deployed method's computational cost.


==> sections/27_solver.tex <==
\subsection{Incorporation into the explicit APIC--MPM solver}
\label{sec:solver}

The offline construction leaves the online material model unchanged. At the start of a time step, the particles already provide the Cauchy stresses to be integrated, and their current positions determine their reconstruction spans. A supplied boundary label follows particle identity: a span containing a labeled boundary particle is not admitted to the full-cell module. Boundary-free classification is an eligibility criterion under this representation, not an independent proof that a sparsely sampled span is completely filled. A boundary-intersected span uses cut quadrature when that module is enabled and its local geometry is admissible; otherwise its complete particle contribution is retained.

Let $\mathcal C_{\full}$, $\mathcal C_{\cut}$, and $\mathcal C_{\mathrm P}$ be the mutually exclusive sets of accepted full cells, accepted cut parents, and cells retaining particle quadrature. The assembled force is
\begin{equation}
 \vct f_i^{\mathrm{AI\text{-}Q}}
 =\sum_{c\in\mathcal C_{\full}}\widehat{\vct f}_{ic}^{\full}
  +\sum_{c\in\mathcal C_{\cut}}\widehat{\vct f}_{ic}^{\cut}
  -\sum_{c\in\mathcal C_{\mathrm P}}\sum_{p\in\mathcal P_c}
                V_p\stress_p\nabla N_i(\vct x_p).
 \label{eq:hybrid}
\end{equation}
An accepted AI parent contributes no standard particle internal force. A rejected cut parent contributes the forces of all its particles and none of its child simplices. This whole-parent decision avoids both duplicate integration and an incomplete replacement. Unsupported particle counts are never accommodated by discarding particles. Geometric rejection is distinguished from invalid inference: an incompatible checkpoint or a nonfinite full-cell prediction is an error condition, not silently reinterpreted as another quadrature rule. Required basis support must be retained in the force assembly; any positive-mass support screening is part of the specified solver branch, not a consequence of the network projection.

The affine particle-in-cell transfers are retained~\cite{Jiang2015,Jiang2017}. Let $t_n$ be the beginning of a step of length $\Delta t$, and let superscript $n$ denote the current particle state. Particle $p$ carries velocity $\vct v_p^n$ and an APIC affine matrix $\mat C_p^n$. Mapping every particle, regardless of integration mode, gives
\begin{equation}
 \begin{aligned}
 m_i^n&=\sum_{p\in\mathcal P}m_pN_i(\vct x_p^n),\\
 \vct p_i^{n,-}
 &=\sum_{p\in\mathcal P}m_pN_i(\vct x_p^n)
       [\vct v_p^n+\mat C_p^n(\vct x_i-\vct x_p^n)].
 \end{aligned}
 \label{eq:p2g}
\end{equation}
Here $\vct x_i$ is the fixed position of grid node $i$ and $\vct p_i^{n,-}$ is its mapped momentum before the force increment. The minus sign in this superscript labels a stage, not a negative momentum. On nodes with $m_i^n>0$, the undamped update is
\begin{equation}
 \vct v_i^{n+1}
 =\frac{\vct p_i^{n,-}}{m_i^n}
  +\frac{\Delta t}{m_i^n}
       [\vct f_i^{\mathrm{AI\text{-}Q},n}+\vct f_i^{\mathrm{ext},n}].
 \label{eq:gridupdate}
\end{equation}
The external-force discretization, prescribed-velocity treatment, loading ramp, and any benchmark-specific damping are the same as in the corresponding baseline calculation. Equation~\eqref{eq:gridupdate} specifies the force substitution in the undamped scheme; it does not introduce a new damping algorithm or an automatic stopping rule.

For transfer back to a particle, define the displacement $\vct d_{ip}^n=\vct x_i-\vct x_p^n$ and the APIC second-moment matrix $\mat D_p^n$. With $\otimes$ denoting the vector outer product, the updates are
\begin{equation}
 \begin{aligned}
 \vct v_p^{n+1}&=\sum_iN_i(\vct x_p^n)\vct v_i^{n+1},\\
 \mat D_p^n&=\sum_iN_i(\vct x_p^n)
                  \vct d_{ip}^n\otimes\vct d_{ip}^n,\\
 \mat C_p^{n+1}&=\left[\sum_iN_i(\vct x_p^n)
              \vct v_i^{n+1}\otimes\vct d_{ip}^n\right](\mat D_p^n)^{-1},\\
 \vct x_p^{n+1}&=\vct x_p^n+\Delta t\vct v_p^{n+1}.
 \end{aligned}
 \label{eq:g2p}
\end{equation}
The sums run over the particle's active nodes. This expression assumes a nonsingular $\mat D_p^n$; a degenerate linear-basis transfer requires the baseline solver's treatment. For the complete quadratic cardinal basis, $\mat D_p^n=(h^2/4)\Id$, where $\Id$ is the identity tensor, recovering the usual factor $4/h^2$ without equating the APIC affine matrix to a constitutive velocity gradient.

The physical velocity gradient is calculated separately from the basis derivatives. Denoting it by $\mat L_p^{n+1}$ gives
\begin{equation}
 \begin{aligned}
 \mat L_p^{n+1}&=\sum_i\vct v_i^{n+1}\otimes\nabla N_i(\vct x_p^n),\\
 \mat F_p^{n+1}&=(\Id+\Delta t\mat L_p^{n+1})\mat F_p^n,\\
 V_p^{n+1}&=\det(\Id+\Delta t\mat L_p^{n+1})V_p^n.
 \end{aligned}
 \label{eq:particlekinematics}
\end{equation}
The particle constitutive law then supplies the subsequent stress and history. Gauss stresses are temporary values used for force integration; they are neither written back as particle stresses nor advanced by a separate constitutive update. The parameters $\theta_{\full}$ and $\theta_{\cut}$ are loaded once, but their geometry-dependent matrices are reevaluated as the particle configurations change.

For a fixed network width, full-cell pair decoding and stress application require $O(P_cQ_{\full})$ and $O(P_cQ_{\full}n_\sigma)$ work, respectively. Cut-cell reconstruction has the corresponding total query count $N_{\simp,c}Q_{\simp}$. The gain sought is improved force accuracy for the available material samples; a wall-time advantage must be established separately after accounting for this additional work. Finally, the known basis assembly preserves zero internal resultant and torque under complete partition-of-unity and linear-precision conditions, as shown in \ref{app:balance}. Those identities do not impose the stronger stress-power pairing needed for an energy-conserving discretization. Consequently, the coupled explicit calculation retains a separately assessed time-step restriction rather than acquiring a stability guarantee from positive Gauss weights alone.

